Visuals Lie, Consistency Speaks: Disentangling Spatial Attention from Reliability in Vision-Language Models

Multimodal Foundation Models are increasingly used as reasoning agents, making reliability, knowing when a model may hallucinate, critical. A common intuition, which we call the Attention-Confidence Assumption, holds that reliability follows from "structural" visual perception: tight attention on relevant regions should signal a trustworthy answer, while scattered attention signals confusion. We challenge this through the VLM Reliability Probe (VRP), a systematic cross-family study of reliability signals in contemporary Vision-Language Models (VLMs). We introduce structural-attention metrics, cluster counts (C_k) and spatial entropy (H_s), to quantify the visual encoder's gaze, and track its evolution (Delta H_s) across layers. This reveals a "Symbolic Detachment": models often "Early Lock" visual features only to diffuse attention later, severing early perception from final generation. Contrary to the grounding hypothesis, we find a "Cluster Failure": spatial attention has near-zero correlation (R approx 0.001) with accuracy. Instead, reliability is a phenomenon of generation dynamics and internal-state distributions. Self-Consistency, the agreement rate across sampled reasoning paths, is the dominant predictor of truth (R = 0.429). Scaling causal interventions exposes a sharp architectural divergence: LLaVA locks its prediction in a fragile late-stage bottleneck, whereas PaliGemma and Qwen2-VL distribute reliability globally, staying resilient even when ~50% or more of their most predictive layer is destroyed. For current VLMs, reliability signals are detached from visual grounding maps and are best inferred from generation-time dynamics and hidden-state probes.

==> figures/reliability_two_panel_combined.tex <==
% Figure 2: Two-panel scientific figure (PGFPlots/TikZ)
% Panel (a): Confidence emergence across processing stages
% Panel (b): Stacked activation profile densities (simulated Gaussians)

\begin{tikzpicture}[font=\sffamily]

% --- Color palette (hex) ---
\definecolor{llavaBlue}{HTML}{1F77B4}
\definecolor{paliOrange}{HTML}{FF7F0E}
\definecolor{successGreen}{HTML}{2CA02C}
\definecolor{failureRed}{HTML}{D62728}
\definecolor{genericGrey}{HTML}{7F7F7F}

% --- Global axis styles ---
\pgfplotsset{
  compat=1.18,
  every axis/.style={
    axis line style={black},
    tick style={black},
    clip=false,
    grid=none,
    label style={font=\bfseries\fontsize{12}{14}\selectfont},
    tick label style={font=\fontsize{10}{12}\selectfont},
    title style={font=\bfseries\fontsize{11}{13}\selectfont},
  }
}

% -------------------------
% Panel (a): line chart
% -------------------------
\begin{axis}[
  name=panelA,
  width=0.49\textwidth,
  height=0.42\textwidth,
  at={(0,0)},
  anchor=south west,
  title={(a) Where Reliability Emerges},
  xlabel={Processing Stage},
  ylabel={Confidence Score},
  xmin=0, xmax=32,
  ymin=0, ymax=11,
  xtick={0,10,20,32},
  xticklabels={Input,Early,Middle,Output},
  ytick={0,2,4,6,8,10},
  enlargelimits=false,
]

% LLaVA: silent phase (0--20) then exponential rise (21--31) ending at 9.2
\addplot[
  very thick,
  llavaBlue,
  samples=200,
  domain=0:32,
] ({x},
  {(
    x<=20
      ? (0.10 + 0.02*sin(deg(3.0*x)) + 0.01*sin(deg(11.0*x)))
      : (
          x<=31
            ? (0.10 + (9.20-0.10) * (exp((x-21)/3.0)-1) / (exp((31-21)/3.0)-1))
            : 9.20
        )
  )}
);

% PaliGemma: fast rise (0--10) then plateau at 10.8
\addplot[
  very thick,
  paliOrange,
  dashed,
  samples=200,
  domain=0:32,
] ({x},
  {(
    x<=10
      ? 10.8*(1-exp(-x/2.2))/(1-exp(-10/2.2))
      : 10.8
  )}
);

% --- Labels on curves ---
\node[font=\bfseries\fontsize{11}{13}\selectfont, text=llavaBlue]
  at (axis cs:28,6.4) {LLaVA};
\node[font=\bfseries\fontsize{11}{13}\selectfont, text=paliOrange]
  at (axis cs:15,10.35) {PaliGemma};

% --- Annotations ---
\draw[->, line width=0.7pt]
  (axis cs:8,2.4) -- (axis cs:15,0.12);
\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=south west]
  at (axis cs:7.6,2.4) {Still Unsure};

\draw[->, line width=0.7pt]
  (axis cs:22.5,10.3) -- (axis cs:28,5.4);
\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=south west]
  at (axis cs:22.0,10.3) {Sudden Decision};

\end{axis}

% -------------------------------------------
% Panel (b): stacked density-style plots
% (Using normalized Gaussian PDFs as a clean
% stand-in for KDE with specified means/stds)
% -------------------------------------------
\begin{groupplot}[
  group style={
    group size=1 by 3,
    vertical sep=0.55em,
  },
  width=0.44\textwidth,
  height=0.14\textwidth,
  at={($(panelA.outer north east)+(1.25em,0)$)},
  anchor=outer north west,
  title={(b) How Neurons Encode Truth},
  xmin=-5, xmax=30,
  ymin=0, ymax=0.25,
  xtick={-5,0,10,20,30},
  ytick=\empty,
  ymajorticks=false,
  axis y line=none,
  axis x line=bottom,
  enlargelimits=false,
  clip=false,
  xlabel={Neuron Activation},
  legend style={font=\fontsize{9}{11}\selectfont, draw=none, fill=none, at={(0.02,0.10)}, anchor=west},
]

% --- Subplot 1: Success neuron ---
\nextgroupplot[
  xticklabels=\empty,
  xlabel=\empty,
]

% Filled: When Right (mean=25, std=2)
\addplot[
  draw=none,
  fill=llavaBlue,
  fill opacity=0.28,
  samples=200,
  domain=-5:30,
]
({x},{1/(2*sqrt(2*pi))*exp(-((x-25)^2)/(2*2^2))})
\closedcycle;

% Dashed: When Wrong (mean=0, std=1)
\addplot[
  very thick,
  failureRed,
  dashed,
  samples=200,
  domain=-5:30,
]
({x},{1/(1*sqrt(2*pi))*exp(-((x-0)^2)/(2*1^2))});

\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=west]
  at (rel axis cs:0.02,0.82) {Success Neuron (e.g., \#1512)};
\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=east]
  at (rel axis cs:0.98,0.82) {Reliability Signal};

\addlegendentry{When Right}
\addlegendentry{When Wrong}

% --- Subplot 2: Failure neuron ---
\nextgroupplot[
  xticklabels=\empty,
  xlabel=\empty,
]

% Filled: When Right (mean=0, std=1)
\addplot[
  draw=none,
  fill=llavaBlue,
  fill opacity=0.28,
  samples=200,
  domain=-5:30,
]
({x},{1/(1*sqrt(2*pi))*exp(-((x-0)^2)/(2*1^2))})
\closedcycle;

% Dashed: When Wrong (mean=20, std=2)
\addplot[
  very thick,
  failureRed,
  dashed,
  samples=200,
  domain=-5:30,
]
({x},{1/(2*sqrt(2*pi))*exp(-((x-20)^2)/(2*2^2))});

\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=west]
  at (rel axis cs:0.02,0.82) {Failure Neuron (e.g., \#1360)};
\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=east]
  at (rel axis cs:0.98,0.82) {Hallucination Signal};

% --- Subplot 3: Generic neuron ---
\nextgroupplot[
]

% Filled: When Right (mean=15, std=3)
\addplot[
  draw=none,
  fill=llavaBlue,
  fill opacity=0.22,
  samples=200,
  domain=-5:30,
]
({x},{1/(3*sqrt(2*pi))*exp(-((x-15)^2)/(2*3^2))})
\closedcycle;

% Dashed: When Wrong (mean=15, std=3)
\addplot[
  very thick,
  failureRed,
  dashed,
  samples=200,
  domain=-5:30,
]
({x},{1/(3*sqrt(2*pi))*exp(-((x-15)^2)/(2*3^2))});

\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=west]
  at (rel axis cs:0.02,0.82) {Generic Neuron};
\node[font=\bfseries\fontsize{10}{12}\selectfont, anchor=east]
  at (rel axis cs:0.98,0.82) {No Signal};

\end{groupplot}

\end{tikzpicture}
